Slot-Level Robotic Placement via Visual Imitation from Single Human Video

The majority of modern robot learning methods focus on learning a set of pre-defined tasks with limited or no generalization to new tasks. Extending the robot skillset to novel tasks involves gathering an extensive amount of training data for additional tasks. In this paper, we address the problem of teaching new tasks to robots using human demonstration videos for repetitive tasks (e.g., packing). This task requires understanding the human video to identify which object is being manipulated (the pick object) and where it is being placed (the placement slot). In addition, it needs to re-identify the pick object and the placement slots during inference along with the relative poses to enable robot execution of the task. To tackle this, we propose SLeRP, a modular system that leverages several advanced visual foundation models and a novel slot-level placement detector Slot-Net, eliminating the need for expensive video demonstrations for training. We evaluate our system using a new benchmark of real-world videos. The evaluation results show that SLeRP outperforms several baselines and can be deployed on a real robot.

==> fig_tex/human_video.tex <==
\begin{figure}[!tbp]
\centering
\includegraphics[width=\linewidth]{figures/human_video.png}
\caption{\textbf{Parsing Human Video.} Show the input on the left, the outputs on the right, and show the detailed pipeline in the middle. Use an example plus text annotations to illustrate, not text/modules only!}
\label{fig:human_video}
\end{figure}

==> fig_tex/robot_view.tex <==
\begin{figure}[!tbp]
\centering
\includegraphics[width=\linewidth]{figures/robot_view.png}
\caption{\textbf{Correlating to the Robot View.} Show the input on the left, the outputs on the right, and show the detailed pipeline in the middle. Use an example plus text annotations to illustrate, not text/modules only!}
\label{fig:robot_view}
\end{figure}

==> fig_tex/supp_test.tex <==
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Text} & \textbf{Image} \\ \hline
% \makecell[t]{First line of text \\ Second line of text} & 
% \makecell[t]{\includegraphics[width=2cm]{example-image}} \\ \hline
% \makecell[t]{Another text entry} & 
% \makecell[t]{\includegraphics[width=2cm]{example-image}} \\ \hline
% \end{tabular}


% \begin{tabular}{c|l}
% \textbf{Verb}   & \textbf{Example}   \\ \hline
% ``goes-to''     & \includegraphics[scale=0.1,valign=c]{example-image-a} \\[1em] \hline
% ``walks-to''    & \includegraphics[scale=0.1,valign=c]{example-image-a}    \\[1em] \hline
% ``says to''     &  \includegraphics[scale=0.1,valign=c]{example-image-a}      \\[1em] \hline
% ``chats to''    &\includegraphics[scale=0.1,valign=c]{example-image-a}
% \end{tabular}

==> section/not-used-5_slotnet.tex <==
\section{\modelName}
\label{sec:slotnet}

\subsection{\modelName for Placement Slot}
\label{subsec:slotnet}
In this section, we describe the details about \modelName architecture and how to generate sythetic training data leveraging SOTA generative AI foundation models.

\input{fig_tex/data_gen}

\input{fig_tex/slotnet}

\vspace{2mm}
\noindent
{\bf Model Architecture.}
Our \modelName architecture is the same as SAM. We finetune SAM, with the start frame of pick-place video as input and the image difference between start and end frame as the prompt.

refer to Figure~\ref{fig:slotnet}




\vspace{2mm}
\noindent
{\bf Training Data Generation.}
There is no large-scale and high-quality existing pick-place data focusing on slot-level pick-place with annotations out there.
% since there are very limited demonstration videos of slot-level pick-place videos out there. 
%
Thus, we decided to create data to find the placement slots for pick-place videos. More details about collection and statistics are in the Supplemental.
%

refer to Figure~\ref{fig:data_gen}


%\vspace{1mm}
%\noindent
%{\it Object-with-slots image collection. }  
We ask people to collect object-centric images of object-with-slots. These images serve as End images and will be used to generate (Start, End) pairs of pick-place videos. Totally, we got \todo{~2K} images spanning \todo{N} categories. 
%
We realized that inpainting is difficult when all slots are full. Thus, we decided to collect images with some empty slots and some full slots.
%
%\vspace{1mm}
%\noindent
%{\it Pick-object Removal.} 
To create the appearance of Start images, which are before the pick-place actions happen, we use inpainting models to remove the pick-object from the slots. We use an SD inpainting model and cleanup.pictures together to get more successful removal results.
%
%\vspace{1mm}
%\noindent
%{\it Slot Mask Annotation.} 
After getting (Start, End) object-centric image pairs, we annotate the slot mask by comparing each paired images using TORAS.
%
%\vspace{1mm}
%\noindent
%{\it Augmentation with Outpainting.} 
To enrich the position of the object-with-slots on canvas and the background appearance, we first randomly transform the objects to a 1024x1024 canvas and then use the generative outpainting method to fill the background appearance with lama-enriched text prompts. The Start object images and Slot masks follow the same transformation to creat (Start, End) full image pairs and GT slot masks. 

%\vspace{1mm}
%\noindent
%{\bf Final Dataset Statistics.}
final data statistics



\vspace{2mm}
\noindent
{\bf Training Details.}



% \input{fig_tex/robot_view}


% \subsection{Correlating to the Single Robot Image}
% \label{subsec:correlate_robot}

% refer to Figure~\ref{fig:robot_view}



==> tab_tex/supp_slerp_results.tex <==
\begin{table*}
    \vspace{-5mm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|p{2cm}|c|c|p{0.3cm}|c|c|}
        
        \hline
        Settings & Video 1 - Start Frame &  Video 1 - End Frame  && Video 2 - Start Frame  &  Video 2 - End Frame \\
        
        \hline
        Different view
        & \includegraphics[scale=0.12, valign=t]{figures/supp/start_pick_place_end/o0-b0-s1-v0/color_000000.jpg}
        & \includegraphics[scale=0.12, valign=t]{figures/supp/start_pick_place_end/o0-b0-s1-v0/color_000220.jpg}
        &
        & \includegraphics[scale=0.12, valign=t]{figures/supp/start_pick_place_end/o0-b0-s1-v1/color_000000.jpg}
        & \includegraphics[scale=0.12, valign=t]{figures/supp/start_pick_place_end/o0-b0-s1-v1/color_000176.jpg}\\


        
        \hline

        
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{More examples for baseline comparisons and our results.}
    \label{tab:slerp_results}
\end{table*}
